Decoherence of Coupled Flip-Flop Qubits Due to Charge Noise

We study the decoherence effect of charge noise on a single flip-flop qubit and two dipole-coupled qubits. We find that a single flip-flop qubit is highly resistant to charge noise at its sweet spots. However, due to the proximity of the charge excited states to the flip-flop logical states, the presence of charge noise greatly reduces the fidelity of two-qubit operations. We identify leakage from the qubit Hilbert space as the main culprit for the reduced gate fidelity. We also explore different bias conditions to mitigate this decoherence channel.

==> figure_tex/__latexindent_temp.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=\textwidth]{figures/two_qubit/Evolution_Time_Frequency_Domains.png}
    \caption{Time evolution for the two qubit system with parameters marked in Figure~\ref{RelaxTime}. The system is initialized to state $\ket{\Psi(0)}=\frac{\sqrt{3}}{2}\ket{01}+\frac{1}{2}\ket{10}$. The top most plots show the time evolution of the system absent any noise while the middle plots include charge noise. The bottom row are the time evolution of $P_{01}$ in the frequency domain. Upward arrows indicate Dirac delta functions. (a) $B=\SI{0.796}{T}$, $E_z-E_c=\SI{3.13}{V/cm}$. This is the location of the single-qubit sweet spot. Without noise, we have gate times of approximately $\SI{150}{ns}$. With noise, we can see that biasing the system to the single-qubit sweet spot is nonideal and quickly decays to its equilibrium state. (b) $B=\SI{0.806}{T}$, $E_z-E_c=\SI{0.95}{V/cm}$.  Moving to the blue band in Figure~\ref{RelaxTime} while trying to maintain fast gate times yields better coherence times but still low fidelity due to the charge leakage. (c) $B=\SI{0.771}{T}$, $E_z-E_c=\SI{0}{}$.  Moving the flip-flop and charge qubits further off-resonance minimizes charge leakage and thus we get excellent coherence times with gate times of approximately $\SI{250}{ns}$.}
    \label{2Q_Evolution}
\end{figure*}

==> figure_tex/dipole_matrix_plot.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/two_qubit/DipoleMatrixPlot.eps}
    \caption{Dipole-dipole Hamiltonian $H_\textrm{dip}$ for parameters $V_{tL}/h = V_{tR}/h = \SI{11.4}{GHz}$, $\omega_{BL}/2\pi=\omega_{BR}/2\pi=\SI{11.15}{GHz}$, and $\epsilon_L/h=\epsilon_R/h= \SI{0}{GHz}$. In constrast to equation~\ref{Hdip}, no terms were neglected. A Schreiffer-Wolff transformation was done to reduce the full $16\times16$ matrix down to a $6\times6$ matrix with states $\ket{00}, \ket{01}, \ket{10}, \ket{11}, \ket{02}, \textrm{ and }\ket{20}$. The first four states form the two-qubit logical basis, while the last two are the dominant leakage states.}
\end{figure}

==> figure_tex/sngle_qubit_charge_dephase.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/single_qubit/1Q_T2_02.png}
\end{figure}

==> figure_tex/two_qubit_evolution.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=\textwidth]{figures/two_qubit/2Q_Evolution.png}
    \caption{Time evolution for the two qubit system with parameters marked in Figure~\ref{RelaxTime}. The system is initialized to state $\ket{\Psi(0)}=\frac{\sqrt{3}}{2}\ket{01}+\frac{1}{2}\ket{10}$. The upper plots show the time evolution of the system absent any noise while the lower plots include charge noise. (a) $B=\SI{0.796}{T}$, $E_z-E_c=\SI{3.13}{V/cm}$. This is the location of the single-qubit sweet spot. Without noise, we have gate times of approximately $\SI{150}{ns}$. With noise, we can see that biasing the system to the single-qubit sweet spot is nonideal and quickly decays to its equilibrium state. (b) $B=\SI{0.806}{T}$, $E_z-E_c=\SI{0.95}{V/cm}$.  Moving to the blue band in Figure~\ref{RelaxTime} while trying to maintain fast gate times yields better coherence times but still low fidelity due to the charge leakage. (c) $B=\SI{0.771}{T}$, $E_z-E_c=\SI{0}{}$.  Moving the flip-flop and charge qubits further off-resonance minimizes charge leakage and thus we get excellent coherence times with gate times of approximately $\SI{250}{ns}$.}
    \label{2Q_Evolution}
\end{figure*}

==> figure_tex/two_qubit_relaxation_90.tex <==
\begin{figure}[htb]
            % Replace figure T_99 and with correct label
            \centering
            \includegraphics[width=\columnwidth]{figures/two_qubit/2Q_T1_0101_9_Large.png}
            \caption{Relaxation time, $T_{90\%}$, computed by setting $F_{01,01}(T_1) = 0.9$. Compared to Figure~\ref{RelaxTime}, we can see that the high coherence band vanishes.}
        \end{figure}

==> long_equations/__latexindent_temp.tex <==
\begin{subequations}
    \begin{align}
        E_0 &= \frac{1}{2}(-\omega_0-\omega_B)-\frac{A}{8} \left(1-\cos \eta\right)-\frac{\Delta\omega_B}{4}\left(1+\cos \eta\right)  \nonumber\\
        &\qquad-\frac{A^2}{16\omega_B}\left((1-\cos\eta)^2+\sin^2\eta(\frac{\omega_B}{4\omega_0}+\frac{\omega_B}{\omega_0+\omega_B}-\frac{\omega_B\Delta\omega_B}{A\omega_0}+\frac{\omega_B\Delta\omega_B^2}{A^2\omega_0})\right)\\
        E_1 &= \frac{1}{2}(-\omega_0+\omega_B)-\frac{A}{8} \left(1-\cos \eta\right)+\frac{\Delta\omega_B}{4}\left(1+\cos \eta\right)\nonumber\\
        &\qquad-\frac{A^2}{16\omega_B}\left(-(1-\cos\eta)^2+\sin^2\eta(\frac{\omega_B}{4\omega_0}+\frac{\omega_B}{\omega_0-\omega_B}+\frac{\omega_B\Delta\omega_B}{A\omega_0}+\frac{\omega_B\Delta\omega_B^2}{A^2\omega_0})\right) \\
        E_2 &= \frac{1}{2}( \omega_0-\omega_B)-\frac{A}{8} \left(1+\cos \eta\right)-\frac{\Delta\omega_B}{4}\left(1-\cos \eta\right)\nonumber\\
        &\qquad-\frac{A^2}{16\omega_B}\left((1+\cos\eta)^2+\sin^2\eta(-\frac{\omega_B}{4\omega_0}-\frac{\omega_B}{\omega_0-\omega_B}+\frac{\omega_B\Delta\omega_B}{A\omega_0}-\frac{\omega_B\Delta\omega_B^2}{A^2\omega_0})\right) \\
        E_3 &= \frac{1}{2}( \omega_0+\omega_B)-\frac{A}{8} \left(1+\cos \eta\right)+\frac{\Delta\omega_B}{4}\left(1-\cos \eta\right)\nonumber\\
        &\qquad-\frac{A^2}{16\omega_B}\left(-(1+\cos\eta)^2+\sin^2\eta(-\frac{\omega_B}{4\omega_0}-\frac{\omega_B}{\omega_0+\omega_B}-\frac{\omega_B\Delta\omega_B}{A\omega_0}-\frac{\omega_B\Delta\omega_B^2}{A^2\omega_0})\right)
    \end{align}
\end{subequations}
